Stockade: Hardware Hardening for Distributed Trusted Sandboxes

The widening availability of hardware-based trusted execution environments (TEEs) has been accelerating the adaptation of new applications using TEEs. Recent studies showed that a cloud application consists of multiple distributed software modules provided by mutually distrustful parties. The applications use multiple TEEs (enclaves) communicating through software-encrypted memory channels. Such execution model requires bi-directional protection: protecting the rest of the system from the enclave module with sandboxing and protecting the enclave module from a third-part module and operating systems. However, the current TEE model, such as Intel SGX, cannot efficiently represent such distributed sandbox applications. To overcome the lack of hardware supports for sandboxed TEEs, this paper proposes an extended enclave model called Stockade, which supports distributed sandboxes hardened by hardware. Stockade proposes new three key techniques. First, it extends the hardware-based memory isolation in SGX to confine a user software module only within its enclave. Second, it proposes a trusted monitor enclave that filters and validates systems calls from enclaves. Finally, it allows hardware-protected memory sharing between a pair of enclaves for efficient protected communication without software-based encryption. Using an emulated SGX platform with the proposed extensions, this paper shows that distributed sandbox applications can be effectively supported with small changes of SGX hardware.

==> Makefile <==
PAPER = exclave
TEX = $(wildcard *.tex)
BIB = references.bib
FIGS = $(wildcard figures/*.pdf figures/*.png graphs/*.pdf graphs/*.png)

.PHONY: all clean diff

all: $(PAPER).pdf

$(PAPER).pdf: $(TEX) $(BIB) $(FIGS) jpaper.cls
	echo $(FIGS)
	pdflatex $(PAPER) </dev/null
	bibtex $(PAPER)
	pdflatex $(PAPER) </dev/null >/dev/null
	pdflatex $(PAPER) </dev/null

#$(CURDIR)/exclave_paper/exclave.tex:
#	rm -rf exclave_paper;
#	git clone https://github.com/ideal8901/exclave_paper.git;
#	cd exclave_paper; \
#	git checkout -b submitted_version_isca2021 origin/submitted_version_micro2021;\
#	cd ..
#
#diff: $(CURDIR)/exclave_paper/exclave.tex
#	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf
#	rm -f ./figures/*-eps-converted-to.pdf
#	rm -f diff.*
#	latexdiff --flatten $< exclave.tex > diff.tex
#	pdflatex diff
#	bibtex diff
#	pdflatex diff
#	pdflatex diff

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf
	rm -f ./figures/*-eps-converted-to.pdf
	rm -f diff.*
	rm -rf exclave_paper


==> multiclient.tex <==
\subsection{Multi Client Isolation}
\label{sec:multiclient}
\begin{figure}[t]
\centering
\includegraphics[width=6.5cm]{figures/futurework.eps}
\vspace{-0.1in}
\caption{Nested Enclave + \Sys architecture}
%\caption{ Secure distributed sandboxes with SGX and bi-enclave}
\label{fig:futurework}
\vspace{-0.1in}
\end{figure}

In app separation of \sys is domain based. 
For multi client requests, \sys serves the requests via multi threading.  
However, client may want to have strongly isolated execution environment even among clients. 
The easiest way to enforce multi client isolation is to launch different bi-enclave per client request.  
On the other hand, \sys can adopt exiting approaches to optimize its memory usage and performance, through sharing.
Chancel~\cite{Chancel} solves the problem with thread isolation and read-only shared memory through binary instrumentation.  
Nested Enclave~\cite{NestedEnclave} introduces shared outer enclaves, among light-weight private inner enclaves via hardware modifications.
Figure ~\ref{fig:futurework} shows futuristic model of \sys, 


==> related.tex <==
\section{Related Work}
\label{sec:related}

%\noindent
%\textbf{Intel SGX:}
%There have been many studies to extend Intel SGX.
%To overcome the lack of trusted libraries and functionalities, user-level system managers have grafted into Intel SGX. 
%Researches~\cite{Haven,scone,graphene-sgx,occlum} suggest trusted library OSes running in the enclave
%enable unmodified application execution in the enclave. 
%%Scone~\cite{scone} shows secure linux container for SGX with narrow and verifiedinterfaces between OS.
%Panoply~\cite{PANOPLY} reduces TCB by applying libc for enclave based on verification after delegation.
%To strengthen security guarantees for SGX,  
%\ju{more works
%Coin Attacks, Autoarkey
%}
%In addition, there are researches~\cite{Eleos,VAULT} that investigate and alleviate the overhead of SGX paging.
%Eleos~\cite{Eleos} shows secure user management memory with minimal enclave exit. 
%Vault~\cite{VAULT} makes integrity verification structure better to alleviate paging overhead.  
%Glamdring~\cite{Glamdring} automates application porting for enclave with annotation and static analysis.

\noindent
\textbf{Sandbox techniques:}
To mitigate vulnerabilities of untrusted codes, numerous studies proposed sandboxing mechanisms~\cite{ostia,SFI, ARMlock, flexdroid, NativeGuard, SDCG, lwCs} 
and commercial products have been released~\cite{NaCl, amazon_sandbox, microsoft_sandbox, yahoo_sandbox, paypal_sandbox_1,paypal_sandbox_2, mozilla_sandbox, chrome_sandbox}.
%There are mainly two kinds of methods for implementing sandbox, fault isolation and process separation.
With controlling memory accesses and syscalls, software-based ~\cite{SFI, NaCl} 
and hardware-based fault isolation~\cite{ARMlock, flexdroid} techniques are proposed.
In addition, isolating untrusted code can be achieved by leveraging the characteristics of a process~\cite{NativeGuard, SDCG, lwCs}.

%Software / Hardware Fault Isolation
% 
% - Efficient SFI~\cite{SFI}, NativeClient~\cite{NaCl}
%
% - ARMlock~\cite{ARMlock}, FlexDroid~\cite{flexdroid}
%
%Process seperation
%
% - NativeGuard~\cite{NativeGuard}, SDCG~\cite{SDCG}, lwCs~\cite{lwCs}

%\noindent
%\textbf{Mutual isolation:}
%The concept of mutual isolation has been studied in TEE.
%Minibox~\cite{Minibox} presents the first two-way sandbox for native x86 code, providing secure file I/O and Iago attack protection. 
%Ryoan~\cite{ryoan} modifies Native Client~\cite{NaCl} to run in enclave.
%Trusted Ryoan module is achieved multi-domain security, providing distributed sandbox, and tag-based secure communication.
%Chancel~\cite{Chancel} proposes multi-client software fault isolation through binary instrumentation and read-only shared memory between threads.
%SGXJail~\cite{SGXJail} shows practical confinement by separating an enclave instance from the other processes
%by confining the enclave process via seccomp filters.
%Several studies accommodate hardware features (Intel MPX or MPK) under software control for multi-domain SFI scheme
%~\cite{occlum, mdSFI, enclavedom, Chancel}.
%Unlike these studies, \sys achieved bi-directional isolation only with simple hardware modification of SGX.

%EnclaveDom~\cite{enclavedom} leverages Intel MPK in the enclave to provide privilege separation within enclave.
%Occlum~\cite{occlum, mdSFI} opensources thier memory safe libOS for Intel SGX along with multi-domain SFI scheme.

\noindent
\textbf{Protected communication:}
%There were prior works reducing communication costs.
%Hotcall~\cite{HotCall}, Switchless call~\cite{switchless} improve ecall/ocall leveraging shared memory to remove mode switching overhead.
%However, they cannot provide a secure channel because it penetrates the non-enclave.
%The channel is not protected, since it is established between enclave and non enclave.
Prior works~\cite{ryoan,PANOPLY} provide inter-enclave secure communication via software-based encryption inherited from SGX.
Other approaches~\cite{occlum,enclavedom} locate all applications within a single enclave and isolate them with runtime library support.
Nested Enclave~\cite{NestedEnclave} presents Multi-Level Security model with hierarchical isolation.
By statically defining a shared sub-enclave, it enables hardware-protected communication via the outer enclave.
Although the outer enclave of Nested enclave can be used for a shared channel among inner enclaves, the outer enclave is a full enclave with
the enclave resource requirement. In addition, one inner enclave can belong to a single outer enclave. Unlike Nested Enclave,
\mbox{\Sys} provides lightweight page-level sharing which allows pairwise connections with multiple enclaves.

%requires at least multiple pages for an outer enclave and
%it only supports statically configured connection at loading time.
%Unlike this, \mbox{\Sys} provides sharing mechanism with single page granularity and dynamically established
%for pairwise lightweight communication with R/W permission.
%}

%\Sys also employs hardware protected communication as well as it supports efficient page-granularity and pairwise dynamic EPC sharing.
%In addition, it provides code generation for security checks and function like interfaces. \thkim{I think it is unnecessary}

